Multi-View Reasoning: Consistent Contrastive Learning for Math Word Problem

Math word problem solver requires both precise relation reasoning about quantities in the text and reliable generation for the diverse equation. Current sequence-to-tree or relation extraction methods regard this only from a fixed view, struggling to simultaneously handle complex semantics and diverse equations. However, human solving naturally involves two consistent reasoning views: top-down and bottom-up, just as math equations also can be expressed in multiple equivalent forms: pre-order and post-order. We propose a multi-view consistent contrastive learning for a more complete semantics-to-equation mapping. The entire process is decoupled into two independent but consistent views: top-down decomposition and bottom-up construction, and the two reasoning views are aligned in multi-granularity for consistency, enhancing global generation and precise reasoning. Experiments on multiple datasets across two languages show our approach significantly outperforms the existing baselines, especially on complex problems. We also show after consistent alignment, multi-view can absorb the merits of both views and generate more diverse results consistent with the mathematical laws.

==> discrimination.tex <==
We optimize a joint probability distribution $P(T,Y|\theta)$ . Since $P(Y|T)=P(T,Y)/P(T)$, we change the $P(T)$ by data augmentation

For discrimination, we also use global shared embedding ($E^{q},E^{op},E^{c}$) to convert the mid-order expressions into embedding sequences, then encode them using two layers GRU, and fuse the text embeddings $E^{w}$ and candidate equation representations $H^{mid\mbox{-}ord}$ by self-attention layer \citep{vaswani2017attention}, and finally calculate the joint probability. This process can be denoted as:
\begin{eqnarray}
H^{mid\mbox{-}ord}_{i}= GRU(Embedding(Y^{mid\mbox{-}ord}_{i})\\
H^{d}_{i}=self\mbox{-}attention(E^{w}_{i},H^{mid\mbox{-}ord}_{i})\\
Prob(T_{i},Y_{i}|\theta) = MLP^{d}(\overline{H^{d}_{i}})\\
\theta = \mathop{argmax}\limits_{\theta} \mathop{E}\limits_{Y_{i}\sim B^{+}} \left[log P(T_{i},Y_{i} | \theta)\right]& \\ \nonumber
- \mathop{E}\limits_{Y_{j}\sim B^{-}} \left[log P(T_{i},Y_{j} |\theta)\right]&
\end{eqnarray}
\indent After learning the joint probability distribution, the algorithm learns a more general symbolic representation, which is also consistent with mathematics rules.
%which in turn enhances the generative and discriminative capabilities.
\subsection{Training and Inference} 
Since it is time-consuming to exhaust all numerical laws in KE Aug-Dis process, we use only use distributive law as external knowledge. We divide the training into two separate processes. In the first phase,  We first transform the labeled mid-order expressions into pre-order and post-order expressions, and then use the teacher force strategy to train both top-down and bottom-up reasoning processes with two order equation, respectively. Simultaneously, we train the consistent contrastive learning process to align the sub-expressions from the two views. KE Aug-Dis process is not involved in training at this phase. In the second phase, we train the KE Aug-dis process separately. During inference, we use the output of the top-down reasoning process $Y^{T2B}$ with beam search strategy as the final prediction in first phase. In second phase, we record the expression $Y^{B2T}$ constructed during the bottom-up reasoning. Then $Y^{T2B}$ and $Y^{B2T}$ are fed into the KE Aug-Dis module together, and then we pick the one with the highest probability as the second phase prediction result:
\begin{eqnarray}
Y^{first-phase}_{i} = Y^{T2B}_{i} \\
Y^{second-phase}_{i} = \mathop{argmax}\limits_{Y \in {Y^{T2B,B2T}}} P(T_{i},Y_{i} | \theta^{*})
\end{eqnarray}
